FlexEmu: Towards Flexible MCU Peripheral Emulation (Extended Version)

Microcontroller units (MCUs) are widely used in embedded devices due to their low power consumption and cost-effectiveness. MCU firmware controls these devices and is vital to the security of embedded systems. However, performing dynamic security analyses for MCU firmware has remained challenging due to the lack of usable execution environments -- existing dynamic analyses cannot run on physical devices (e.g., insufficient computational resources), while building emulators is costly due to the massive amount of heterogeneous hardware, especially peripherals. Our work is based on the insight that MCU peripherals can be modeled in a two-fold manner. At the structural level, peripherals have diverse implementations but we can use a limited set of primitives to abstract peripherals because their hardware implementations are based on common hardware concepts. At the semantic level, peripherals have diverse functionalities. However, we can use a single unified semantic model to describe the same kind of peripherals because they exhibit similar functionalities. Building on this, we propose FlexEmu, a flexible MCU peripheral emulation framework. Once semantic models are created, FlexEmu automatically extracts peripheral-specific details to instantiate models and generate emulators accordingly. We have successfully applied FlexEmu to model 12 kinds of MCU peripherals. Our evaluation on 90 firmware samples across 15 different MCU platforms shows that the automatically generated emulators can faithfully replicate hardware behaviors and achieve a 98.48% unit test passing rate, outperforming state-of-the-art approaches. To demonstrate the implications of FlexEmu on firmware security, we use the generated emulators to fuzz three popular RTOSes and uncover 10 previously unknown bugs.

==> acknowledgments.tex <==
\section*{Acknowledgement}


==> listings/dma-llm-res.tex <==
\begin{listing}[H]
\begin{minted}[
breakanywhere,
baselinestretch=1.0,
numbersep=2pt,
bgcolor=bgcolor,
fontsize=\scriptsize,
breaklines,
highlightcolor=highlightcolor,
]{json}
{
  "trans_descs": [
    {
      "enable": {
        "enable": {"register": "Channel_0_CCR", "field": "EN", "value": "0x01"},
        "disable": {"register": "Channel_0_CCR", "field": "EN", "value": "0x00"}
      },
      "complete_evt": {
        "irq_idx": "0",
        "happen": {"register": "ISR", "field": "TCIF1", "value": "0x01"},
        "active": {"register": "Channel_0_CCR", "field": "TCIE", "value": "0x01"},
        "enable": {"register": "Channel_0_CCR", "field": "TCIE", "value": "0x01"},
        "disable": {"register": "Channel_0_CCR", "field": "TCIE", "value": "0x00"},
        "clear": {"register": "IFCR", "field": "CTCIF1", "value": "0x01"}
      },
      "src": "Channel_0_CMAR",
      "src_width": {
        "register": "Channel_0_CCR", "field": "MSIZE",
        "value_map": {"0x00": "1", "0x01": "2", "0x02": "4"}
      },
      "dst": "Channel_0_CPAR",
      "dst_width": {
        "register": "Channel_0_CCR", "field": "PSIZE",
        "value_map": {"0x00": "1", "0x01": "2", "0x02": "4"}
      },
      "cnt": "Channel_0_CNDTR",
      "dir": {"register": "Channel_0_CCR", "field": "DIR", "value": "0x01"}
    },
    ...
  ]
}
\end{minted}
\small
% \vspace{-1em}
\caption{\textbf{Part of the LLM's response for the prompt generated from the DMA model.}}
\label{lst::dma-llm-res}
\end{listing}

==> listings/dma-template.tex <==
\begin{listing}[H]
\begin{minted}[
breakanywhere,
baselinestretch=1.0,
numbersep=2pt,
bgcolor=bgcolor,
fontsize=\scriptsize,
breaklines,
highlightcolor=highlightcolor,
]{json}
{
  // a list of transfer descriptors
  "trans_descs": [
    {
      // when to enable the channel
      "enable": {
        "enable": {
          "reg": "<register name>", "field": "<field name>", "value": "<value of the field>",
        },
        "disable": {
          "reg": "<register name>", "field": "<field name>", "value": "<value of the field>",
        },
        "active": {
          "reg": "<register name>", "field": "<field name>", "value": "<value of the field>",
        },
      },
      // the event generated when the transfer completes
      "complete_evt": {
        "happen": {
          "reg": "<register name>", "field": "<field name>",
          "value": "<when the event happens, the field is set to this value>",
        },
        "active": {
          "reg": "<register name>", "field": "<field name>",
          "value": "<when the event is enabled, the field is set to this value>",
        },
        "enable": {
          "reg": "<register name>", "field": "<field name>",
          "value": "<the event interrupt is enabled when this value is written into the field>",
        },
        "disable": {
          "reg": "<register name>", "field": "<field name>",
          "value": "<the event interrupt is disabled when this value is written into the field>",
        },
        "clear": {
          "reg": "<register name>", "field": "<field name>",
          "value": "<the event happen flag is cleared when this value is written into the field>",
        },
      },
      "src": "<the register holding DMA transfer source address>",
      // the register field representing source transfer chunk width (in bytes)
      "src_width": {
        "reg": "<register name>", "field": "<field name>",
        "value_map": {"<field value>": "<mapped value>", ...},
      },
      "dst": "<the register holding DMA transfer destination address>",
      // the register field representing destination transfer chunk width (in bytes)
      "dst_width": {
        "reg": "<register name>", "field": "<field name>",
        "value_map": {"<field value>": "<mapped value>", ...},
      },
      "cnt": "<the register holding the number of data to be transferred>",
      // [OPTIONAL] the register field representing transfer direction
      "dir": {
        "reg": "<register name>", "field": "<field name>", "value": "<field value>",
      },
    },
    ...,
  ],
},
\end{minted}
\small
% \vspace{-1em}
\caption{\textbf{JSON-like template generated using the DMA model.}}
\label{lst::dma-template}
\end{listing}
